ChartEditBench: Evaluating Grounded Multi-Turn Chart Editing in Multimodal Language Models

While Multimodal Large Language Models (MLLMs) perform strongly on single-turn chart generation, their ability to support real-world exploratory data analysis remains underexplored. In practice, users iteratively refine visualizations through multi-turn interactions that require maintaining common ground, tracking prior edits, and adapting to evolving preferences. We introduce ChartEditBench, a benchmark for incremental, visually grounded chart editing via code, comprising 5,000 difficulty-controlled modification chains and a rigorously human-verified subset. Unlike prior one-shot benchmarks, ChartEditBench evaluates sustained, context-aware editing. We further propose a robust evaluation framework that mitigates limitations of LLM-as-a-Judge metrics by integrating execution-based fidelity checks, pixel-level visual similarity, and logical code verification. Experiments with state-of-the-art MLLMs reveal substantial degradation in multi-turn settings due to error accumulation and breakdowns in shared context, with strong performance on stylistic edits but frequent execution failures on data-centric transformations. ChartEditBench, establishes a challenging testbed for grounded, intent-aware multimodal programming.

==> Chapters/Abstracts/abstract_v3.tex <==
% ChartBench Abstract
% To be included in main paper via \input{abstract}

While Multimodal Large Language Models (MLLMs) have achieved remarkable success in one-shot visualization generation, they frequently overlook the iterative nature of real-world exploratory data analysis. In practice, users refine charts through progressive updates, a process that requires maintaining code-visual consistency across multiple turns. To bridge this gap, we introduce \textbf{ChartBench}, a comprehensive benchmark formalized to evaluate incremental, visually grounded chart code editing. Unlike existing static benchmarks, ChartBench assesses models on multi-turn modification chains, comprising 5,000 difficulty-controlled instances and a rigorous human-verified subset. We propose a robust evaluation framework that mitigates the instability of standard LLM-as-a-Judge metrics by integrating execution-based fidelity, pixel-level visual similarity, and logical code verification. Experiments with state-of-the-art MLLMs reveal a significant performance degradation in multi-turn settings due to error accumulation, with a marked disparity between stylistic updates (where models perform well) and data-centric transformations (where execution failures are prevalent). ChartBench establishes a challenging testbed for advancing conversational visual programming agents, shifting the focus from static generation to dynamic, state-aware editing.

==> Chapters/Chapter1_Introduction.tex <==
\section{Introduction}
\label{Chapter 1}



==> Chapters/Chapter1_Introduction_Refined.tex <==
\section{Introduction}
\label{Chapter 1}

Recent work on multimodal large language models (MLLMs) has driven rapid progress on \emph{chart generation}: given a natural language description or an input image, models learn to produce plotting code or new charts, supported by large synthetic corpora and dedicated benchmarks. This generation-centric view has yielded impressive results for one-shot tasks, but it overlooks a core aspect of how charts are used in practice. Developers, analysts, and technical writers rarely create a visualization once; instead, they iteratively refine an existing code base, adjusting encodings, adding statistical overlays, or reformatting layouts based on new requirements and feedback. Editing an existing chart specification is therefore a natural, high-value capability for MLLM-based assistants, yet it remains comparatively underexplored.

Existing benchmarks only partially touch this space. ChartQA~\cite{masry2022chartqa} and PlotQA~\cite{methani2020plotqa} evaluate question answering over static charts, treating visualizations as read-only artifacts rather than editable programs. Chart-to-code systems focus on reconstructing code from a final image or generating code from natural language, typically in a single turn and often without explicit control over task difficulty. These settings do not directly test whether models can reason about the \emph{difference} between two visual states and apply precise, minimal edits to the underlying code, nor do they provide fine-grained levers for probing how performance changes with modification complexity or interaction length.

\textbf{Our key contributions are:}
1. We formalize \emph{incremental chart code editing} as a benchmark task where a model updates chart code from an initial code–plot pair and a target plot or natural language delta.\\
2. We build \textbf{ChartEditBench}, a difficulty-controlled synthetic dataset of 5{,}000 instances across 12 modification types, including a 430-example human-verified subset.\\
3. We introduce visually grounded metrics that jointly assess rendering success, visual similarity, and code semantics, providing more reliable scores than generic LLM-based judges for analyzing chart-editing behavior.



==> Chapters/Chapter3_Dataset_Collection.tex <==
% Chapter Template
\section{Dataset Description} % Main chapter title

\label{Chapter3} % Change X to a consecutive number; for 


